The Evolution of Quantum Secure Direct Communication: On the Road to the Qinternet

Communication security has to evolve to a higher plane in the face of the threat from the massive computing power of the emerging quantum computers. Quantum secure direct communication (QSDC) constitutes a promising branch of quantum communication, which is provably secure and overcomes the threat of quantum computing, whilst conveying secret messages directly via the quantum channel. In this survey, we highlight the motivation and the status of QSDC research with special emphasis on its theoretical basis and experimental verification. We will detail the associated point-to-point communication protocols and show how information is protected and transmitted. Finally, we discuss the open challenges as well as the future trends of QSDC networks, emphasizing again that QSDC is not a pure quantum key distribution (QKD) protocol, but a fully-fledged secure communication scheme.

==> README <==
LaTeX package: forest [2017/07/14 v2.1.5 Drawing (linguistic) trees]

Copyright (c) 2012-2017 Saso Zivanovic
                   (Sa\v{s}o \v{Z}ivanovi\'{c})
saso.zivanovic@guest.arnes.si


ABSTRACT

`forest' is a pgf/tikz-based package for drawing linguistic (and other
kinds of) trees. Its main features are:
- a packing algorithm which can produce very compact trees;
- a user-friendly interface consisting of the familiar bracket
encoding of trees plus the key--value interface to option-setting;
- many tree-formatting options, with control over option values of
individual nodes and mechanisms for their manipulation;
- a powerful mechanism for traversing the tree;
- the possibility to decorate the tree using the full power of pgf/tikz;
- an externalization mechanism sensitive to code-changes.


LICENSE

This work may be distributed and/or modified under the
conditions of the LaTeX Project Public License, either version 1.3
of this license or (at your option) any later version.
The latest version of this license is in

http://www.latex-project.org/lppl.txt

and version 1.3 or later is part of all distributions of LaTeX
version 2005/12/01 or later.


For the list of files constituting the work see the main source file
of the package, `forest.dtx', or the derived `forest.sty'.


